Performance Estimation of Synthesis Flows cross Technologies using LSTMs and Transfer Learning

Due to the increasing complexity of Integrated Circuits (ICs) and System-on-Chip (SoC), developing high-quality synthesis flows within a short market time becomes more challenging. We propose a general approach that precisely estimates the Quality-of-Result (QoR), such as delay and area, of unseen synthesis flows for specific designs. The main idea is training a Recurrent Neural Network (RNN) regressor, where the flows are inputs and QoRs are ground truth. The RNN regressor is constructed with Long Short-Term Memory (LSTM) and fully-connected layers. This approach is demonstrated with 1.2 million data points collected using 14nm, 7nm regular-voltage (RVT), and 7nm low-voltage (LVT) FinFET technologies with twelve IC designs. The accuracy of predicting the QoRs (delay and area) within one technology is $\boldsymbol{\geq}$\textbf{98.0}\% over $\sim$240,000 test points. To enable accurate predictions cross different technologies and different IC designs, we propose a transfer-learning approach that utilizes the model pre-trained with 14nm datasets. Our transfer learning approach obtains estimation accuracy $\geq$96.3\% over $\sim$960,000 test points, using only 100 data points for training.

==> abstract.tex <==
{\it\bf Abstract -} 
This paper presents an advanced DAG-based algorithm for datapath synthesis that targets area minimization using logic-level resource sharing. The problem of identifying common specification logic is formulated using unweighted graph isomorphism problem, in contrast to a weighted graph isomorphism using AIGs. In the context of gate-level datapath circuits, our algorithm solves the unweighted graph isomorphism problem in linear time.  The experiments are conducted within an industrial synthesis flow that includes the complete \textit{high-level synthesis}, \textit{logic synthesis} and \textit{placement and route} procedures. Experimental results show a significant runtime improvements compared to the existing datapath synthesis algorithms. 


%Datapath synthesis is one the most critical optimization problems encountered in the modern design flow. Datapath synthesis techniques have been mainly discussed in the context of traditional high-level synthesis research, such as \textit{resource sharing}, \textit{scheduling} and \textit{binding}, relied on Data Flow Graph (DFG) representation. %However, this is limited to constructability of DFGs and the function of operators. 
%Recently, applying high-level optimization technique, such as \textit{resource sharing} has been applied in logic synthesis, using Directed acyclic graph (DAG)-based techniques implemented using \textit{And-Inv-Graphs} (AIGs). These techniques overcome some limitation of resource sharing encountered traditional datapath synthesis for standard-cell designs. This paper presents an advanced DAG-based algorithm that targets area minimization using logic-level resource sharing. We formulate the problem of identifying common specification logic using \textit{unweighted graph isomorphism}, in contrast to a weighted graph isomorphism problem using AIGs. We demonstrate that our technique can significantly 1) reduce both area and delay, or 2) reduce area without delay overhead, for large industry datapath designs, including 64-bit multipliers. The results are conducted in an industry synthesis flow that includes the complete high-level synthesis. logic synthesis procedures, which demonstrates that the proposed approach provides unique improvements. Experimental results show a significant runtime improvement compared to the existing algorithm. In the context of gate-level datapath circuits, our algorithm solves the unweighted graph isomorphism problem in \textit{linear} time. 

\keywords{Logic synthesis, datapath synthesis, resource sharing, graph isomorphism}
